R3DS: Reality-linked 3D Scenes for Panoramic Scene Understanding

We introduce the Reality-linked 3D Scenes (R3DS) dataset of synthetic 3D scenes mirroring the real-world scene arrangements from Matterport3D panoramas. Compared to prior work, R3DS has more complete and densely populated scenes with objects linked to real-world observations in panoramas. R3DS also provides an object support hierarchy, and matching object sets (e.g., same chairs around a dining table) for each scene. Overall, R3DS contains 19K objects represented by 3,784 distinct CAD models from over 100 object categories. We demonstrate the effectiveness of R3DS on the Panoramic Scene Understanding task. We find that: 1) training on R3DS enables better generalization; 2) support relation prediction trained with R3DS improves performance compared to heuristically calculated support; and 3) R3DS offers a challenging benchmark for future work on panoramic scene understanding.

==> fig/fig-fine-category-plot.tex <==
\begin{figure}
\centering
\setkeys{Gin}{width=0.85\linewidth}
\begin{tabularx}{\textwidth}{Y@{\hspace{1mm}} Y@{\hspace{1mm}}}
% \multicolumn{2}{c}{\textbf{RGB}} & \multicolumn{2}{c}{\textbf{Depth}} \\
\includegraphics{fig/images/category_plot_fine_chair.pdf}
\subcaption{Chair}\label{fig:category_plot_chair}
& 
\includegraphics{fig/images/category_plot_fine_sofa.pdf}
\subcaption{Sofa}\label{fig:category_plot_sofa}
\\
\includegraphics{fig/images/category_plot_fine_table.pdf}
\subcaption{Table}\label{fig:category_plot_table}
& 
\includegraphics{fig/images/category_plot_fine_lighting.pdf}
\subcaption{Lighting}\label{fig:category_plot_lighting}
\\
% \multicolumn{2}{c}{\includegraphics{fig/images/obj_sizes.png}
% }\subcaption{Object sizes}
% \includegraphics{fig/images/obj_sizes.png}\subcaption{Object sizes}
% \\
\end{tabularx}
\caption{
Histograms of the fine-grained categories for `Chair', `Sofa', `Table' and 'Lighting'.
There are a variety of object instances in our scenes.
Note that lighting objects are also found in dramatically different support relations with the architecture and other objects (e.g., table lamp vs ceiling lamp vs floor lamp).
}
% \label{fig:region_type_plot}
% \vspace{-12pt}
\end{figure}

==> fig/fig-interface-custom-masks.tex <==

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{fig/images/adding_custom_mask.pdf }
\caption{
The interface allows annotators to insert objects even if there are no corresponding masks for them. 
}
\label{fig:custom_masks}
\end{figure}


==> fig/fig-object-support-plot.tex <==

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{fig/images/object_support_plots.pdf}
\caption{
\textbf{Object Statistics Plots.}
\textit{Object-to-architecture support}: shows various support relations between objects and architecture elements (floor, wall, ceiling). The circle radius indicates the average number of the object type supported by a given arch type per panorama, whereas the color indicates the number of times the object type is supported by that arch type out of the total number of times the object type appears. For example, we see that on average, same number of bookcases can be found on the floor and the wall in a panorama, but overall bookcases appear more on the floor than on the wall.
\textit{Object-to-region}: 
\textit{Object-to-object support}: 
}
\label{fig:obj_support_plot}
\end{figure*}


==> fig/fig-regionType-objectCategory-plot.tex <==

% \begin{figure}[b!]
% \centering
% \includegraphics[width=\linewidth]{fig/images/region_type_plot.pdf}
% \caption{
% Histogram of all region (i.e. room) types in our \dataset dataset.
% The three most common region types are bedroom, bathroom and hallway, but there is a long-tail distribution with many other region types.
% }
% \label{fig:region_type_plot}
% \end{figure}


\begin{figure}
\centering
\setkeys{Gin}{width=\linewidth}
\begin{tabularx}{\textwidth}{Y@{\hspace{1mm}}}
% \multicolumn{2}{c}{\textbf{RGB}} & \multicolumn{2}{c}{\textbf{Depth}} \\
\includegraphics[width=0.65\linewidth]{fig/images/region_type_plot.pdf}
\captionof{figure}{Histogram of all region (i.e. room) types in our \dataset dataset.
The three most common region types are bedroom, bathroom and hallway, but there is a long-tail distribution with many other region types.}\label{fig:region_type_plot} \\

\includegraphics[width=0.65\linewidth]{fig/images/category_plot_coarse.pdf} 
\captionof{figure}{\textbf{Coarse Object Categories.} Histogram of the 20 most common object categories in \dataset. We see that the scenes in our dataset exhibit a long-tail distribution over common object categories occurring in real-world scenes.}\label{fig:category_plot}
\\
\end{tabularx}
% \caption{
% Histogram of all region (i.e. room) types in our \dataset dataset.
% The three most common region types are bedroom, bathroom and hallway, but there is a long-tail distribution with many other region types.
% }
% \label{fig:region_type_plot}
\end{figure}


==> sections/05-applications.tex <==
\section{Other Applications}

\TODO{Mention potential applications in the motivation or conclusion.}

\subsection{Single-view Shape Retrieval}
Given a RGB image of real object, the goal is to retrieve a 3D shape from database that match the object geometry presented in image. The input includes image, object mask and 3D shapes. We output a list of ranked 3D shapes in descending order of similarity in the joint-embedding space. To compute view-dependent metrics, we also need shape pose annotations. We represent 3D shapes as multiview renderings. 

\textbf{Benchmark methods}
\begin{itemize}
    \item \textbf{CMIC}: Single Image 3D Shape Retrieval via Cross-Modal Instance and Category Contrastive Learning
    \item \textbf{generalizable CMIC}: Generalizing Single-View 3D Shape Retrieval to Occlusions and Unseen Objects
\end{itemize}

These two methods share the same model architecture, but differ from training strategy. CMIC only trains on the small target datasets, but generalizable CMIC first trains on large-scale synthetic dataset and then fine-tune on small realistic data that demonstrate better performance. We can compare retrieval results using models trained on small real data (Pix3D, Scan2CAD), synethtic data (MOOS) and RLSD. Note that RLSD would contain more object categories available and we need to count the actual number in annotation files. For provided 3D shapes for annotation, We have 28 general categories and 139 fine-grained categories, comparing to 9 categories in Pix3D and 4 categories in MOOS.

Note that the RLSD CAD annotation also enables voxel-based shape retrieval for MP3D scene mesh like Scan2CAD. One of variants we can perform is multi-view shape retrieval as we may observe the same object from multiple viewpoints. But one concern is that the CAD annotations across different viewpoints could be inconsistent.

\subsection{Single-view Object Pose Estimation}

Given a RGB image of real object, we aim to estimate pose of the object. We can estimate only the orientation or the full 6DoF pose? The input is usually an image along with an associated 3D shape if the model requires templates. The output are three Euler angles and position for 6DoF pose estimation. We can obtain shape pose annotations including orientations and positions from sceneState JSON files.

\textbf{Benchmark methods} (need to update literature survey)
\begin{itemize}
    \item \textbf{Pose from Shape}: Deep Pose Estimation for Arbitrary 3D Objects
    \item \textbf{PoseContrast}: Class-Agnostic Object Viewpoint Estimation in the Wild with Pose-Aware Contrastive Learning (No 3D shape knowledge required)
    \item \textbf{Templates for 3D Object Pose Estimation Revisited}: Generalization to New Objects and Robustness to Occlusions
    \item \textbf{Gen6D}: Generalizable Model-Free 6-DoF Object Pose Estimation from RGB Images
    \item \textbf{MegaPose}: 6D Pose Estimation of Novel Objects via Render \& Compare
\end{itemize}

Recent progress in single-view object pose estimation focuses on generalizing to novel objects and potential occlusions. We can either train and compare models directly on RLSD data or use models pretrained on other datasets to test generalizability on RLSD data as we have diverse object categories. Those methods can be roughly divided into two groups, with or without 3D shape knowledge. 

Not sure whether pose information is introduced solely by RLSD because oriented bounding box for object instance mesh is also available in MP3D.

\subsection{Single-view Scene Generation}
By combining single-view shape retrieval and object pose estimation, we can perform single-view scene generation that retrieves and aligns 3D CAD models from a shape database to an input image. The input includes image, object instance masks and 3D shapes. For each object, we estimate its 6DoF pose and retrieve the best matching 3D shape

\textbf{Benchmark methods}
\begin{itemize}
    \item \textbf{Mask2CAD}: 3D shape prediction by learning to segment and retrieve
    \item \textbf{Patch2CAD}: patchwise embedding learning for in-the-wild shape retrieval from a single image
    \item \textbf{ROCA}: Robust CAD model retrieval and alignment from a single image
    \item \textbf{Total3DUnderstanding}: Joint Layout, Object Pose and Mesh Reconstruction for Indoor Scenes from a Single Image
    \item \textbf{InstPIFu}: Towards High-Fidelity Single-view Holistic Reconstruction of Indoor Scenes
\end{itemize}

Depending on the quality and density of RLSD annotations, we may produce more cluttered synthetic scene from a single view than what Scan2CAD provide because we purse more object categories.


==> sections/unused/annotation-interface.tex <==
\subsection{Annotation interface}
\label{sec:supp-annotation-interface}
The core idea behind the system is that having panoramas, camera poses, and 3D architecture allows us to insert 3D assets into the scene while \textbf{visually overlaid} on the panorama wrapped on a sphere.
Compared against \cite{maninis2023cad}, this lets the user pick and place 3D CAD models directly on to the panorama and facilitates matching the shapes. We implement two viewing modes, panorama mode and architecture mode, to let users switch between overlaid panorama and underlying 3D scene (see Figure~\ref{fig:rlsd_interface}).
% We use a 3D annotation interface which shows a panorama of a room and ask annotators to select and place 3D object models to best match the panoramic image.

\mypara{Design Goals.}
It is non-trivial to design an annotation system for synthetic 3D scenes that perfectly reproduce real world appearance regarding geometry and texture. Considering limited 3D shapes we possess, we develop a system that build scenes satisfying the following goals: 
\textit{1). Correct correspondence between 2D objects and 3D shapes}. This allows downstream tasks such as 3D object detection and potential applications in embodied AI.
\textit{2). Semantic-matched 3D shape selection}. It is crucial for the image-based 3D shape retrieval task and discuss more about it in Sec~\ref{sec:annotation-interface} in detail. 
\textit{3). Visually-matched 3D shape manipulation}. 3D shapes inserted into the scene should respect the position, scale, and orientation of their counterparts in the panoramas, so as to be a globally reasonable digital twin of input imagery.
\textit{4). Physically-plausible objects placement}. In particular, objects should be in physical contact with other objects or the architecture, not floating in space or penetrating with each other. 
% This contact information facilitates use of the output scenes in downstream tasks involving physical simulation.

In practice, it is impossible to exhaustively create a perfect CAD reconstruction of the input imagery due to finite size of 3D shape repositories.
We identify areas where we decide to sacrifice fidelity in order to keep the system feasible:
\textit{1). Mismatch on surface appearance between 3D shapes and the corresponding visual instances}. This relaxation allows more flexible use of a finite set of CAD models while still enforcing that the output be a geometrically plausible scene.
\textit{2). Mismatch on scene complexity}. It's difficult to obtain instance segmentations at super fine-grained detail, and it will weight an undue burden on annotators to label all possible objects. We predefine 32 object classes from Matterport3D mask labels.

\mypara{Data Assets}
In general, the annotation system requires as input image and architecture data, where each data item consists of a floorplan plus a set of panoramic images within the floorplan, along with their camera locations w.r.t the floorplan. Floorplan can be formulated as raster image indicating house structures as line segments, %,that are metrically scaled, , room type labels of each room, and icons indicating placement of appliances.
or decomposed architecture parameters of each wall, floor and ceiling specifying location and scale. We demonstrate the functionality of the system on Matterport3D~\cite{chang2017matterport3d}.
We obtain each RGB panoramas by stitching 6 skybox images from the same camera viewpoint. During the data preprocessing stage, we also parse panoramas into semantic object instance masks as the minimal annotation unit. Segmentations can be assumed as prerequisite, or be computed automatically using learning-based methods \cite{he2027maskrcnn}. In our case, we directly render segmentations from Matterport3D's annotated instance house meshes. Instead of reconstructing only one room layout from floorplan at once, we build whole house-level architecture containing dozens of rooms from Matterport3D with manual clean-up. 

\mypara{Workflow.}
We describe a typical annotation workflow starting with any empty scene.
A user freely pan the camera to explore the whole scene while the overlay is kept in sync (\textit{Goal \#1}).
By clicking an object to be annotated, it brings up a list of sorted 3D shapes of the same category as the object based on shape similarity.
The user is expected to identify the best matching 3D shape that satisfies \textit{Goal \#2}. The initialized pose of inserted 3D shape is automatically calculated based on pose suggestion by a learning-based method on backend and where the mouse was clicked. The user can further manipulate the position, scale, and orientation of objects to satisfy \textit{Goal \#3}. The placement is attached to a specific surface already in the scene, which satisfies \textit{Goal \#4}.
% The system maintains link between the selected object and 3D shape, satisfying \textbf{Goal \#1}.
Figure~\ref{fig:rlsd_system} illustrates the overview of the pipeline.


\input{fig/fig-many2many-feat}
\mypara{Mask-to-Object Assignment}
In some cases, it is overly restrictive to assume that there is a one-to-one correspondence between masks and objects.
For example, an object may need to be assigned to multiple masks because the two masks correspond to parts of the same object, separated by occlusion.
In certain other occasions, we have masks that include multiple objects (See Figure~\ref{fig:rlsd_many2many_feat}).
Our system supports these cases such that a user can place multiple models for the same mask by re-selecting a mask that already has a model already assigned and then inserting a new model. For cases where a model is shared among multiple masks, the user first insert the model having selected one of the masks. Then, the user can assign other relevant masks to that model.


\input{fig/fig-object-similarity}
\mypara{Object Selection.} 
To address the challenge of retrieving 3D shape from single-view object image, we deploy a simple but effective approach based on the light field descriptor \TODO{cite}, called \textit{Shape Sorter} (see Figure~\ref{fig:rlsd_system}). As a pre-computation, we render 100 views for each 3D shape by placing the cameras at the vertices of 10 predefined dodecahedrons and looking towards the object's centroid. Then we compute a light field descriptor for each view to form a shape representation of 3D shape. During inference, after pre-filtering a set of 3D shapes with the same general category as the target object, we compute the  Euclidean distance of descriptors between an object mask and each 3D shape view as their similarity. A list of sorted 3D shapes in ascending order in distance is returned.
We decompose the requirement on semantically-matching objects into 4 sub-aspects: category, shape, structural and functional similarities. For example, a category mismatch constitutes a `chair' being annotated with a `table', a shape mismatch constitutes `high-back armchair' being annotated with a `dining-chair', a structural mismatch constitutes a `single-seater chair' being annotated with a `double-seater chair' and a functional mismatch constitutes a `an armchair with no wheels' being annotated with a `swivel chair with wheels and no arms' (refer \Cref{fig:obj_similarity}). \todo{Compared to prior work, we exclude door and window objects for annotations since they are represented as holes on walls in architecture.}
% Placed CAD models should match the category (e.g. chair) and shape (e.g. cushioned sofa chair, wood chair) of their corresponding object in the panoramas.

\input{fig/fig-object-alignment}

\mypara{Object Alignment.} 
Manipulating 3D shapes in terms of position, orientation and scale to correctly visually match target objects is time-consuming. As our system physically attaches placed objects to a supporting surface, we only allow one rotational degree of freedom that can be adjusted (i.e. rotation about the object's up direction).
To automatically suggest an appropriate pose for a newly-inserted object, we leverage a learning-based pose estimation approach, PoseContrast~\cite{xiao2021posecontrast}, called \textit{Pose Suggester} in the system (see Figure~\ref{fig:rlsd_system}). It tackles the 6DoF object pose estimation problem using contrastive learning without aware of 3D shape knowledge.
The objects are aligned to the images as closely as possible. Additionally, the objects have two types of support structure: object-to-object support and object-to-architecture support. The Object-to-object support ensures that two objects are supported by each other properly. For example, a microwave should be placed on a counter and not hanging mid-air. The object-to-architecture support, on the other hand, ensures that an object is supported by the correct architecture element (floor, wall or ceiling). For example, a chest of drawers is more likely to be placed on the floor than on the wall (refer \Cref{fig:obj_alignment}). 
\todo{
% Discuss more about Figure~\ref{fig:scene_hierarchy}. 
For annotated scene hierarchy, what kind of information does 3D scene graph of prior work have? What's difference compared to them.}

\mypara{Custom Masks.} We further enable add annotations of objects for which there are no masks to ensure the scenes are heavily cluttered and objects are properly supported. 
In some cases, the user may decide to leave a mask unannotated.
This could be because the mask is invalid or, there are no viable models for the object.
In this case, the user can mark the object as `unannotated' and leave comments for the reason.


==> sections/unused/other-applications.tex <==
\section{Applications}

\subsection{Single-view Shape Retrieval}
Given a RGB image of real object, the goal is to retrieve a 3D shape from database that match the object geometry presented in image. The input includes image, object mask and 3D shapes. We output a list of ranked 3D shapes in descending order of similarity in the joint-embedding space. To compute view-dependent metrics, we also need shape pose annotations. We represent 3D shapes as multiview renderings. We can obtain image-shape annotations from sceneState JSON files.

\textbf{Benchmark methods}
\begin{itemize}
    \item \textbf{CMIC}: Single Image 3D Shape Retrieval via Cross-Modal Instance and Category Contrastive Learning
    \item \textbf{generalizable CMIC}: Generalizing Single-View 3D Shape Retrieval to Occlusions and Unseen Objects
\end{itemize}

These two methods share the same model architecture, but differ from training strategy. CMIC only trains on the small target datasets, but generalizable CMIC first trains on large-scale synthetic dataset and then fine-tune on small realistic data that demonstrate better performance. We can compare retrieval results using models trained on small real data (Pix3D, Scan2CAD), synethtic data (MOOS) and RLSD. Note that RLSD would contain more object categories available and we need to count the actual number in annotation files. For provided 3D shapes for annotation, We have 28 general categories and 139 fine-grained categories, comparing to 9 categories in Pix3D and 4 categories in MOOS.

Note that the RLSD CAD annotation also enables voxel-based shape retrieval for MP3D scene mesh like Scan2CAD. One of variants we can perform is multi-view shape retrieval as we may observe the same object from multiple viewpoints. But one concern is that the CAD annotations across different viewpoints could be inconsistent.

\subsection{Single-view Object Pose Estimation}

Given a RGB image of real object, we aim to estimate pose of the object. We can estimate only the orientation or the full 6DoF pose? The input is usually an image along with an associated 3D shape if the model requires templates. The output are three Euler angles and position for 6DoF pose estimation. We can obtain shape pose annotations including orientations and positions from sceneState JSON files.

\textbf{Benchmark methods} (need to update literature survey)
\begin{itemize}
    \item \textbf{Pose from Shape}: Deep Pose Estimation for Arbitrary 3D Objects
    \item \textbf{PoseContrast}: Class-Agnostic Object Viewpoint Estimation in the Wild with Pose-Aware Contrastive Learning (No 3D shape knowledge required)
    \item \textbf{Templates for 3D Object Pose Estimation Revisited}: Generalization to New Objects and Robustness to Occlusions
    \item \textbf{Gen6D}: Generalizable Model-Free 6-DoF Object Pose Estimation from RGB Images
    \item \textbf{MegaPose}: 6D Pose Estimation of Novel Objects via Render \& Compare
\end{itemize}

Recent progress in single-view object pose estimation focuses on generalizing to novel objects and potential occlusions. We can either train and compare models directly on RLSD data or use models pretrained on other datasets to test generalizability on RLSD data as we have diverse object categories. Those methods can be roughly divided into two groups, with or without 3D shape knowledge. 

Not sure whether pose information is introduced solely by RLSD because oriented bounding box for object instance mesh is also available in MP3D.

\subsection{Single-view Scene Generation}
By combining single-view shape retrieval and object pose estimation, we can perform single-view scene generation that retrieves and aligns 3D CAD models from a shape database to an input image. The input includes image, object instance masks and 3D shapes. For each object, we estimate its 6DoF pose and retrieve the best matching 3D shape

\textbf{Benchmark methods}
\begin{itemize}
    \item \textbf{Mask2CAD}: 3D shape prediction by learning to segment and retrieve
    \item \textbf{Patch2CAD}: patchwise embedding learning for in-the-wild shape retrieval from a single image
    \item \textbf{ROCA}: Robust CAD model retrieval and alignment from a single image
    \item \textbf{Total3DUnderstanding}: Joint Layout, Object Pose and Mesh Reconstruction for Indoor Scenes from a Single Image
    \item \textbf{InstPIFu}: Towards High-Fidelity Single-view Holistic Reconstruction of Indoor Scenes
\end{itemize}

Depending on the quality and density of RLSD annotations, we may produce more cluttered synthetic scene from a single view than what Scan2CAD provide because we purse more object categories.



\subsection{Room Layout Estimation}

\textbf{Related work}
\begin{itemize}
    \item \textbf{LayoutNet}: Reconstructing the 3D Room Layout from a Single RGB Image
    \item Manhattan Room Layout Reconstruction from a Single 360 image: A Comparative Study of State-of-the-art Methods
    \item Holistic 3D Scene Understanding from a Single Image with Implicit Representation
\end{itemize}

\subsection{Panoramic Scene Understanding}
As mentioned in previous weekly meeting by Angel, given an input panorama, the goal is to output 3D bounding boxes of
the room and all major objects inside, together with their semantic categories such that a 3D room reconstruction can be built.

\textbf{Related work}
\begin{itemize}
    \item \textbf{PanoContext}: A Whole-room 3D Context Model for Panoramic Scene Understanding
    \item \textbf{DeepPanoContext}: Panoramic 3D Scene Understanding with Holistic Scene Context Graph and Relation-based Optimization
\end{itemize}

RLSD system leverages panoramas to facilitate image-to-3D-shape annotation, but we don't introduce direct panoramic-wise annotations for panoramic scene understanding. It seems the original MP3D data provides enough information to do this particular task. Not sure if it deserves more investigation.


\subsection{Generative Scene Synthesis}
Training on artist-designed well-furnished room, the goal is to learn a probabilistic generative model capable of sampling rooms conditioned on room layouts with novel object arrangements for retrieved 3D shapes. Different from scene generation methods that only output new synthesized rendering views, this line of directions aims to produce a 3D scene mesh composed of separate object meshes that enables further manipulation including object removal, completion, re-arrangement and interaction.

\textbf{Related work}
\begin{itemize}
    \item \textbf{Sceneformer}: Indoor scene generation with transformers
    \item \textbf{ATISS}: Autoregressive Transformers for Indoor Scene Synthesis
    \item \textbf{DiffuScene}: Scene Graph Denoising Diffusion Probabilistic Model for
Generative Indoor Scene Synthesis
\end{itemize}

Previous work mainly use 3D-Front data to train and test their approaches.

==> tab/data_compare_quality.tex <==
\begin{table*}[t!]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}l c ccc c cc@{}}
        \toprule
         \multirow{2}{*}{Dataset} & \multirow{2}{*}{\thead{Object\\Shape\\Match}} & \multicolumn{3}{c}{Object Alignment} & & \multicolumn{2}{c}{Scene Completeness}
         \\
         \cmidrule(l{0pt}r{2pt}){3-8}
         & & \thead{Object-to-Image\\Alignment} & \thead{Object-to-Object\\Alignment} & \thead{Object-to-Support\\Structure \\(wall/floor/ceiling)\\Alignment} & & \thead{Objects\\per scene} & \thead{Object categories\\per scene}
         \\
         \midrule
         Scan2Cad & Good & Excellent & Poor & N/A & & Poor & Poor \\
         Pix3D & Excellent & Excellent & N/A & N/A & & N/A & N/A \\
         ScanCadObjSim & Good & Excellent & N/A & N/A & & Poor & Poor \\
         % \textbf{RLSD} & Good & Excellent & Good & Good & & Excellent & Excellent \\
         \textbf{RLSD} & Good & 38.2 (IoU) & Good & Good & & 21 & 8 \\
         \bottomrule
    \end{tabular}}
    \caption{\textbf{Dataset Comparison.} Rating Scale: Poor, Average, Good, Excellent. \emph{(RLSD row needs to be revised.)} \qw{As discussed in the meeting, we won't have a big tow-column table. We probably describe it in the text instead.}}
    \label{tab:data_compare_quality}
\end{table*}


==> tab/data_compare_stats_v0.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}lcccccccccc@{}}
        \toprule
             \multirow{2}{*}{Datasets}  & \multirow{2}{*}{\#Houses} & \multirow{2}{*}{\#Rooms} & \multirow{2}{*}{\#Panoramas} & \multirow{2}{*}{\thead{\#Unique\\CAD models}} & \multirow{2}{*}{\thead{\#Object\\Categories}} & \multirow{2}{*}{\thead{\#Annotated\\Objects}}    & \multicolumn{2}{c}{\thead[c]{Object instances\\per view}} & \multicolumn{2}{c}{\thead[c]{Object Categories\\per view}}
         \\
         \cmidrule(l{0pt}r{2pt}){8-9}
         \cmidrule(l{0pt}r{2pt}){10-11}
         
          &&&&&& &Avg & Max & Avg & Max \\
         \midrule

        
        CAD-Estate & &12,000 &&12,429 &49 & &5.2 &47 &3.4 & 15 \\

        % Pix3D \\
         Scan2Cad & &1506 & &3049 &9 &14,225 &9.4 &40 &4.1 & 13 \\

         \midrule
        % Replica-Pano \\
        Replica-CAD &1 &&&&&&22 &87 &14 &43 \\
        % HSSD \\
        3DFront &&18,968 & &16,563 &34 &101,997 &7 &23 &5.4 &13 \\

        \midrule
        
        iGibson-DPC &15& && &57 &500 &18 &49 & 10 & 24 \\

        \midrule
        
        \textbf{RLSD (Ours)} &20 &&808 &3807 &110 (78 coarse) &19,495 &38 &171 &10 (9 coarse) &24 (22 coarse) \\
        
         \bottomrule
    \end{tabular}}
    \caption{\textbf{RLSD statistics.} 
    % s\qw{"Object instances per pano" is not precise here.} 
    }
    \label{tab:data_compare_stats-v0}
\end{table*}


==> tab/heu_support_rel.tex <==
\begin{table}
\centering
% \resizebox{\linewidth}{!}
{
\begin{tabular}{@{}l cccc@{}}
\toprule
Relations & Accuracy & Precision & Recall & F1  \\
\midrule
obj-floor & 0.74 & 0.95 & 0.59 & 0.73  \\
obj-ceil & 0.98 & 0.04 & 0.04 & 0.04  \\
obj-wall & 0.97 & 0.88 & 0.74 & 0.80  \\
obj-obj & 0.97 & 0.16 & 0.99 & 0.28  \\
\bottomrule
\end{tabular}
}
% \vspace{-6pt}
\caption{
The support relation classification results of applying the heuristic relation predictor to the ground-truth support annotations of \dataset.
}
\label{tab:heu_support_rel}
\end{table}
